Angle of Arrival Estimation Using SRS in 5G NR Uplink Scenarios

This paper presents a comprehensive exploration of Angle of Arrival (AoA) estimation techniques in 5G environments, using the Sounding Reference Signal (SRS) in Uplink scenarios both in simulations and with actual measurements. Leveraging 5G capabilities, we investigate AoA algorithms for single-base station positioning. The study includes simulations and practical tests on a developed dedicated testbed featuring a base station equipped with a three-element Uniform Linear Array (ULA), considering Line of Sight conditions in an open environment. The testbed, employing Ettus E312 as the transmitter and Ettus N310 as the receiver, details waveform structures and reception processes. Additionally, our study examines the performance of Angle of Arrival (AoA) estimation algorithms, such as Multiple Signal Classification (MUSIC), Estimation of Signal Parameters via Rotational Invariant Techniques (ESPRIT), and Joint Angle and Delay Estimation (JADE) ESPRIT. A MATLAB ray tracing propagation model of the environment where the measurements are conducted, has been constructed. Simulation results using this model are presented, along with the actual measurements. The obtained results affirm the effectiveness of our implementation.

==> Data/aoa_15m.tex <==
1	1.87025055014844	2.27333333333334	2.26458414110330	1.84553379364851	2.10800000000000	2.37304408286910
2	1.82814805006152	2.23250000000000	2.22543269835708	1.74739565717886	2.09200000000000	2.09800946772660
3	1.67820630531719	2.08800000000000	2.07900893376842	1.92874982361340	1.97400000000000	2.05452028639370
4	1.89902109672312	2.30400000000000	2.29415480637784	1.91418967353955	1.99000000000000	1.97874745387193
5	1.56376725097670	1.97000000000000	1.96522763757588	1.94071556389317	2.01000000000000	1.99746210349158
6	1.81935947127633	2.23200000000000	2.22524534226339	1.82071614773292	1.90000000000000	1.88628021325885
7	1.58752126544070	1.99600000000000	1.98809808420751	1.87819701704070	1.95600000000000	1.94113365842772
8	1.63797125618929	2.06200000000000	2.05616990292507	1.97723498034663	2.05250000000000	2.04011947695977
9	1.74250574351002	2.18200000000000	2.15048115518826	1.88303717768710	1.96500000000000	1.94991223690661
10	1.85042742541659	2.23500000000000	2.22869076412043	1.88722203299385	1.96400000000000	1.95231257543664
11	1.71041207140823	2.12800000000000	2.11844362179665	1.95520495367800	1.99600000000000	1.97394090386235
12	1.78809094376167	2.21200000000000	2.20580909777991	1.83827708901045	1.91200000000000	1.89976068520708
13	1.77630504529972	2.19000000000000	2.14331406500144	1.90508936499642	1.98000000000000	1.97050766078362
14	1.68360024032422	2.09600000000000	2.09119203048724	1.95346499023936	2.02600000000000	2.01436730577514
15	1.60658103349534	2.01400000000000	2.00705748071712	1.92466984515052	1.99400000000000	1.98258880461619
16	1.58342198235176	1.99333333333333	1.98565063130634	1.91323293802072	1.99000000000000	1.97649712100387
17	1.41991601587746	1.82250000000000	1.81673136145705	1.92094945597373	1.99250000000000	1.98281559881792
18	1.85991862174050	2.27200000000000	2.26546650765051	2.04205245231080	2.11600000000000	2.10348516772921
19	1.68608760410121	2.08200000000000	2.07782889770916	1.93177858202513	1.99600000000000	1.99543036817738
20	1.64291252687284	2.04800000000000	2.04371192187855	1.98057129529130	2.05600000000000	2.04211510121998
21	1.66937266343148	2.08000000000000	2.07381047533980	1.91183022968113	1.98600000000000	1.97594505428209
22	1.71073720947846	2.11600000000000	2.11350968858022	1.85281628668548	1.93250000000000	1.92015874801198
23	1.72687921232279	2.14000000000000	2.13414912369538	1.95587024704258	2.02800000000000	2.01297897248117
24	1.72459183956422	2.13200000000000	2.12938354169565	1.95722087511150	2.02000000000000	2.01211978038462
25	1.70342256871020	2.11000000000000	2.10314165386888	1.96045830626674	2.03000000000000	2.01600307778752
26	1.75907228284041	2.16800000000000	2.16433644756114	1.88803147934798	1.96800000000000	1.95207618747900
27	1.70064837659380	2.11000000000000	2.10120596018158	1.96808021321109	2.04000000000000	2.02673934410446
28	1.46998468317519	1.86000000000000	1.85424022854884	1.84554764911812	1.87000000000000	1.82014296794470
29	1.70743827249834	2.10400000000000	2.09625575595166	1.88605610601200	1.96400000000000	1.94844563500592
30	1.28757512270777	1.69200000000000	1.68602144790243	1.90782822532943	1.98000000000000	1.96724714422026
31	1.74137058151922	2.15800000000000	2.15162570779462	1.90040516059217	1.97000000000000	1.96068999001402
32	1.59309752828103	2.00200000000000	1.99652583854334	1.85039657520269	1.92800000000000	1.91388428110958
33	1.67259999423497	2.08200000000000	2.07474250542676	1.95836431217784	2.03000000000000	2.01695005333055
34	1.67411218490591	2.08400000000000	2.07628789812007	1.93788446496542	2.01500000000000	2.00150147482349
35	1.53172996763232	1.93800000000000	1.93029250786477	1.86716780811719	1.94200000000000	1.92947423309025
36	1.80161126907521	2.21400000000000	2.20817640660614	1.88446476249747	1.95750000000000	1.94432302209203
37	1.73491304919731	2.14000000000000	2.13379172515325	1.80775716166638	1.88800000000000	1.87485515904607
38	1.67238682019966	2.08000000000000	2.07643681421200	1.85826599282572	1.93000000000001	1.92133885436232
39	1.83972264401286	2.26750000000000	2.26188666406906	1.85865970403259	1.93000000000001	1.91788894872050
40	2.08226917820990	2.54400000000000	2.53693279710081	1.94323013496632	2.01000000000001	1.99750384725478
41	1.76751839586456	2.17400000000000	2.13640441713489	1.80791812836733	1.89000000000000	1.87819572613294
42	1.80101590156016	2.22250000000000	2.21820895474797	1.86271498645973	1.93800000000000	1.92561331588200
43	1.62328477416524	2.04800000000000	2.04465065363261	1.87186120366482	1.93000000000000	1.91674774401424
44	1.67877643901046	2.11000000000000	2.10635575433345	1.88955098970084	1.95999999999999	1.94821670299956
45	1.64623307503646	2.09600000000000	2.09158922697674	1.89584498410737	1.97000000000000	1.95597754026396
46	1.15237795830447	1.56333333333333	1.55634600044087	1.87434955313765	1.94200000000000	1.92990696506243
47	1.39121341153823	1.78600000000000	1.78085705868203	1.91668724364919	1.99800000000000	1.98599906180514
48	1.25811931851690	1.66000000000000	1.65389758648125	1.82143346584894	1.90200000000000	1.90070920733375
49	1.94014524348390	2.36800000000000	2.36111276185581	1.88104652720601	1.96200000000000	1.94876396147252
50	1.81151603698219	2.21600000000000	2.21237468693829	1.81211699600679	2.05400000000000	2.02927415431864
51	1.26828309761556	1.63400000000000	1.62448378652775	1.83192720087061	1.91200000000000	1.89785530270125
52	1.71688974712561	2.12200000000000	2.11688613394301	1.84010770766648	1.92000000000000	1.90570954536501
53	1.72871407682385	2.14750000000000	2.13542547489566	1.89274600044526	1.97400000000000	1.95760776505970
54	1.58539323020659	1.97600000000000	1.96813098104909	1.94195739132148	2.01600000000000	2.00479144658254
55	1.83260184131136	2.24600000000000	2.23864393946490	1.84332947669591	1.92000000000000	1.90472152875405
56	1.68596304019848	2.08400000000000	2.07786513688844	1.76997401280348	1.90400000000000	1.89166815485702
57	1.59196995932446	1.98000000000000	1.97140588107714	1.83198918147172	1.91200000000000	1.89807269609104
58	1.59594648979112	1.98200000000000	1.97438833395317	1.91171536169272	1.97000000000000	1.96872729999910
59	1.32790896791271	1.70200000000000	1.69578832649117	1.87396904127933	1.94800000000000	1.93618479655867
60	1.36708219024696	1.75750000000000	1.75080629625903	1.93261145784447	2.00600000000000	1.99374228537327

==> Data/aoa_50m.tex <==
1	-0.657092589431837	-0.819999999999999	-0.852733740618154	-1.06114445072043	-1.23000000000000	-1.21670431910141
2	-0.784636297478460	-0.926666666666672	-0.951014592865543	-1.12930643092113	-1.31600000000000	-1.30384069243517
3	-0.898099810851231	-1.09800000000000	-1.13096794382252	-1.19303001861056	-1.40800000000000	-1.39356746523276
4	-0.436941214995768	-0.619999999999999	-0.646485027196791	-1.04008695078641	-1.22200000000000	-1.20661259177615
5	-0.385873593913400	-0.547499999999996	-0.562780566102444	-1.15106400309871	-1.36000000000000	-1.34509214710628
6	-0.467710222345471	-0.646000000000001	-0.660689413195442	-1.19398726815358	-1.41400000000000	-1.40277182800594
7	-0.810105867737923	-0.990000000000001	-1.00876560193626	-1.23411054653364	-1.46200000000000	-1.44673458007128
8	-0.283631820867204	-0.500000000000000	-0.527310888079904	-1.34336895017308	-1.52600000000000	-1.51783861043289
9	-0.958822383167551	-1.18000000000000	-1.21196026463504	-1.25896411774550	-1.48200000000000	-1.48072848583569
10	-0.466780618295215	-0.666000000000000	-0.694066087287061	-1.14240260244681	-1.35400000000000	-1.34939646840701
11	-0.573033169844026	-0.749999999999997	-0.781635422029771	-1.12774729880995	-1.34800000000000	-1.34223163235195
12	-0.462949510238087	-0.657999999999998	-0.698655438412782	-1.18072526966915	-1.41666666666667	-1.40923708898535
13	-0.531446924101314	-0.658000000000004	-0.694696441819148	-1.19696439915725	-1.37200000000000	-1.36634405049252
14	-0.745912752060467	-0.880000000000001	-0.916847698610940	-0.973686119148375	-1.17400000000000	-1.16525322478986
15	-0.793763938642408	-0.916000000000000	-0.956915838093373	-1.07076487654934	-1.32000000000000	-1.30736665452833
16	-1.10807333216500	-1.29400000000000	-1.33015839088043	-1.06525196663403	-1.30600000000000	-1.29433018864929
17	-1.00737121164147	-1.16000000000000	-1.19940362625406	-1.12956249124200	-1.36400000000000	-1.35400828946060
18	-0.876058898205331	-1.01400000000000	-1.04616143587201	-1.02101286122528	-1.25200000000000	-1.24174929101508
19	-0.770943236246235	-0.930000000000003	-0.967358591195898	-1.00443091086724	-1.22500000000000	-1.20880258352581
20	-0.665652173565438	-0.802500000000002	-0.823486592573076	-0.851920823858463	-1.06800000000000	-1.05473021169161
21	-0.463478654053064	-0.565999999999997	-0.597569985586557	-0.772501579681833	-0.952499999999997	-0.952096927316527
22	-0.596487813362056	-0.738000000000002	-0.775974832123631	-0.953437025419332	-1.16800000000000	-1.15351002973291
23	-0.461470031728964	-0.598000000000002	-0.633434094337993	-1.00726753896179	-1.22800000000000	-1.21950213798077
24	-0.545566287292699	-0.655999999999997	-0.696368472525330	-1.05306750635265	-1.28000000000000	-1.26521174609103
25	-0.390298582143158	-0.524000000000001	-0.573366190076058	-1.29714660596760	-1.50800000000000	-1.49835357230262
26	-0.428606292405262	-0.566000000000000	-0.602708979309096	-1.02291389620777	-1.21750000000000	-1.20612004848303
27	-0.621147434286259	-0.775999999999999	-0.817436137306286	-1.05867703024170	-1.27600000000000	-1.26062462756213
28	-0.525730781306026	-0.636000000000001	-0.675864075277752	-1.10780294499012	-1.31800000000000	-1.30627050103334
29	-0.630250012329133	-0.801999999999998	-0.836423333598142	-1.31496322006078	-1.54200000000000	-1.52921006040957
30	-0.845614550803649	-0.995999999999998	-1.02993530778970	-1.34313768838774	-1.56250000000000	-1.55106061281328
31	-0.940668414314018	-1.08666666666667	-1.13055933323739	-1.23808529011153	-1.45200000000000	-1.43904822329502
32	-0.783424451593753	-0.976000000000002	-1.00364025424806	-1.05893212831354	-1.25400000000000	-1.24297040655272
33	-1.00728880110642	-1.17800000000000	-1.20202390104427	-1.21256867669560	-1.41400000000000	-1.40220435034893
34	-0.948360351349365	-1.11250000000000	-1.13343599892963	-1.04299735026762	-1.24600000000000	-1.23433007316860
35	-0.937738119874356	-1.12200000000000	-1.14887468893646	-1.02092714705421	-1.21600000000000	-1.20156723622855
36	-0.845107130946173	-1.00200000000000	-1.02208459755978	-0.896840844938556	-1.08666666666667	-1.07837678111864
37	-0.808313806412478	-0.966000000000000	-0.992313927402935	-1.07734672872371	-1.27400000000000	-1.26262641935087
38	-0.859640858240878	-1.05000000000000	-1.07531797471847	-1.16728499814036	-1.39000000000000	-1.38065083957049
39	-0.565468725121748	-0.728000000000003	-0.750151425346038	-1.09669669857907	-1.30750000000000	-1.29362642261469
40	-0.473693315511149	-0.626000000000002	-0.656465619402882	-1.18560553651600	-1.40000000000000	-1.39123136261556
41	-0.467080884922066	-0.602000000000004	-0.633926517605430	-1.06778894788003	-1.26666666666667	-1.25420564476881
42	-0.648543125548007	-0.802000000000001	-0.836991575700681	-1.18562168799790	-1.39800000000000	-1.38617038285544
43	-0.738221090632521	-0.892000000000002	-0.914587956783039	-1.13070898342253	-1.34000000000000	-1.32294323265462
44	-0.796520314590731	-0.956000000000000	-0.976698322829130	-1.27416150397768	-1.48400000000000	-1.47234156030434
45	-0.733020293581868	-0.876000000000002	-0.903994657864297	-1.23259044172139	-1.44400000000000	-1.43341821897681
46	-1.07391822083617	-1.24400000000000	-1.28051856487117	-1.30076383941327	-1.52200000000000	-1.51354924974514
47	-1.00189002127644	-1.18750000000000	-1.18774464885383	-1.02619010467367	-1.22600000000000	-1.21409670961148
48	-0.871619131980918	-1.04000000000000	-1.08568613474180	-1.26229846751732	-1.46000000000000	-1.44918079220392
49	-0.955092488383249	-1.12400000000000	-1.17318371992937	-1.12837721951070	-1.32600000000000	-1.31408054390207
50	-0.867327512148262	-1.02000000000000	-1.06099080529069	-1.15025190935778	-1.34200000000000	-1.33046764027934
51	-1.09801078055663	-1.28000000000000	-1.31192212691113	-1.08784112904892	-1.27500000000000	-1.26550630319074
52	-1.06758039709251	-1.25800000000000	-1.30249964597302	-1.12983426262005	-1.34400000000000	-1.32784187143760
53	-1.08449180470008	-1.27600000000000	-1.31453930979383	-1.09393490713952	-1.30200000000000	-1.28475417283162
54	-1.02367581048028	-1.27000000000000	-1.31977779603854	-1.09709982272345	-1.31200000000000	-1.29949306412357
55	-1.28712847340131	-1.50750000000000	-1.54570348522425	-1.19773966257703	-1.38000000000000	-1.36789903617322
56	-1.07522324226087	-1.28000000000000	-1.29776948783341	-0.946418674899564	-1.13000000000000	-1.11915038283188
57	-1.05092102715673	-1.22800000000000	-1.26849238118223	-1.17617064640162	-1.39400000000000	-1.38221284871619
58	-0.813559580759941	-0.949999999999999	-1.00113855209036	-1.14264228623269	-1.35000000000000	-1.33558446750900
59	-1.19498509705919	-1.38000000000000	-1.39437685393940	-1.25642299366183	-1.46800000000000	-1.45607620389008
60	-0.846149769721264	-0.974000000000001	-1.00170493019099	-1.06979017123535	-1.24500000000000	-1.23742168888606

==> Data/ray_tracing_parking_sims_2_4_v2.tex <==
10 0.189845697897213 0.189878881541420 0.189893660080172
15 0.117481325396962 0.117310016271775 0.117264601829705
20 0.090845116255540 0.090332563893583 0.090745839192735
25 0.027534235722354 0.027382847727912 0.026445268806182
30 0.642320744419852 0.641665852260273 0.641415182653144
35 0.040660577633551 0.040304432721428 0.040021822011450
40 0.023237809023253 0.023544067772262 0.023318799463965
45 0.033688513180323 0.033356969026678 0.033699180828907
50 0.034471512219035 0.034643284038693 0.034627553132420

==> Data/ray_tracing_parking_sims_3_5_v2.tex <==
10 0.140417666783307 0.140796601629066 0.140157722335624
15 0.234079696569725 0.233890605489099 0.233808314711180
20 0.0895809503488648 0.0891251713714418 0.0892974719485907
25 0.072911222196164 0.072134022197599 0.072244721490985
30 0.642219922031806 0.641583431301289 0.641582480600476
35 0.035382503836200 0.034333835840143 0.034630102925209
40 0.022833556556821 0.022434017114110 0.021671400579108
45 0.577479917405953 0.577418859937018 0.576736401414448
50 0.011769174873382 0.010930247830371 0.011282080473017

==> Data/sigid3.tex <==
1	2.02219956361754	1.99400000000000	1.99273440632903	6.23552649524281	5.65250000000000	5.61548350435578	9.70729159402790	9.16000000000000	9.17574350872337	18.2837792321641	18.6700000000000	18.6717153294872	20.7804100391829	21.0860000000000	21.1017018527934	23.1213781109538	23.7925000000000	23.8760970003489	43.3290376547919	44.7720000000000	44.9982779738644
2	1.31862658775019	1.26500000000000	1.25910448833268	6.43991884319740	5.82000000000000	5.82558780374522	9.26870060650070	8.74800000000000	8.74598714280206	17.1692305898399	17.6100000000000	17.6092375798955	20.3950362408151	20.8866666666667	20.8858460703999	23.7461806724172	24.2720000000000	24.3199274743446	43.8831872249171	43.6920000000000	43.8864293368579
3	1.70278417060368	1.62000000000000	1.62593512697588	6.94588067253750	6.28400000000000	6.36414982137099	8.73999061929821	8.25000000000000	8.23898375013553	17.5866930262823	17.9240000000000	17.9385125024653	19.7897653432990	20.3260000000000	20.3338468818385	23.6962482392035	24.2280000000000	24.2848074333069	42.6319947055123	45.0280000000000	45.2650257706624
4	1.57805615529248	1.48250000000000	1.49288824956599	6.88467114864518	6.46500000000000	6.48863509568476	9.00545587791062	8.47200000000000	8.44484522838851	18.6069258075204	19.0920000000000	19.1052476247615	20.3041177027709	20.6250000000000	20.6259515226498	23.8870208734893	24.6060000000000	24.6365706531701	43.0216469073335	45.1366666666667	45.2605985427814
5	1.81873502673108	1.74800000000000	1.75355154302154	6.94270654237066	6.47800000000000	6.56086412238719	8.88752863788909	8.49750000000000	8.49747030431526	17.2727743247242	17.5825000000000	17.5836874893169	19.5262931027587	19.9375000000000	19.9376926193105	23.6623105627113	24.1960000000000	24.2241125301081	42.3474402066113	44.0320000000000	44.1112860196460
6	1.82703686256434	1.73000000000000	1.72713540859821	5.94411830027913	5.52500000000000	5.53818858361565	9.36088206649371	8.97200000000000	8.96785424399174	20.8791514191048	21.5950000000000	21.6053855308438	19.8276356360308	20.2600000000000	20.2845959163722	23.0488925717765	23.5900000000000	23.6465825574323	43.7586886816272	46.2150000000000	46.3529451259554
7	1.54424813042315	1.44800000000000	1.44683394717160	6.15656190235104	5.67800000000000	5.69949075339553	10.4230104776226	9.91200000000000	9.93294738582108	17.2086178101674	17.9875000000000	17.9396752377176	20.2417344216364	20.6525000000000	20.6793730240244	24.1887812362166	24.6500000000000	24.6367018506929	40.6796430511252	44.7225000000000	44.8355962632956
8	1.73278293669209	1.67400000000000	1.68961056451793	6.09718511345272	5.63600000000000	5.67738440876105	10.4295383396845	9.83333333333333	9.86867228148257	18.4944187598171	19.2560000000000	19.2372102557457	19.4448083764934	19.8880000000000	19.9165624415639	23.8415919760057	24.2875000000000	24.3528892215916	42.2910539050524	45.2080000000000	45.3821044161311
9	2.13359778083550	2.06000000000000	2.08026991524891	5.85161970767980	5.33000000000000	5.37187612913983	10.6621543320290	9.96400000000000	10.0310435642084	20.5284332110444	20.8540000000000	20.9195193216851	20.1555558160596	20.5940000000000	20.6140273668353	23.5282541106648	24.0120000000000	24.1096470782892	44.1023846939355	46.1825000000000	46.5518484152864
10	2.65635528849397	2.61000000000000	2.60929201666735	5.36768563086643	4.70750000000000	4.80208677747237	9.54100494507177	8.59333333333333	8.66587434911650	16.4178333546117	17.1050000000000	17.0568219844665	19.9690273969045	20.3920000000000	20.4116278744978	23.8973693663187	24.3425000000000	24.3800395505764	44.4062254671945	45.1760000000000	45.3987463191320
11	2.77807408608402	2.79000000000000	2.79427332765282	5.75373530338159	5.15000000000000	5.20535758766728	8.76514618111490	7.51400000000000	7.63713410639093	15.6774697353008	16.1680000000000	16.1440318105827	20.0491114078667	20.4340000000000	20.4455028627725	23.5681979581299	24.1800000000000	24.2326908144116	44.3205872696536	46.1880000000000	46.5308907371229
12	2.04856875219291	2.04600000000000	2.05042181266875	4.85285348641393	4.19800000000000	4.20515557742482	8.05539362177127	7.58600000000000	7.66753787698207	16.8545090180980	17.4860000000000	17.4534386451647	20.4217039805288	21.0020000000000	21.0365735612784	23.3668599240371	23.9220000000000	23.9089516100778	43.4833996361875	45.0225000000000	45.4017520393097
13	1.79846187748127	1.80000000000000	1.79765996798916	5.22997735399911	4.43200000000000	4.53988096937303	8.24632281266524	7.50750000000000	7.58038701471730	18.4699839368179	19.1050000000000	19.1425277508109	20.1605467406308	20.8420000000000	20.9055352979639	23.7164683230365	24.3780000000000	24.4131193238629	42.2507949367298	45.0120000000000	45.1056741528924
14	1.50810202694230	1.50000000000000	1.50068153658130	6.15602088038813	5.46000000000000	5.58592961499708	10.3096496006911	9.80200000000000	9.83728446124667	16.8330912797095	17.1580000000000	17.1585539806862	19.7817967114459	20.1280000000000	20.1654129756767	24.5054109694369	24.9925000000000	25.0941211720260	40.6114175277243	44.9033333333333	45.0934254358235
15	2.02733098297460	2.01800000000000	2.01663997946980	6.22231593264163	5.63000000000000	5.67859545486234	10.0889056554396	9.62600000000000	9.65865463716940	17.7363176343688	18.2640000000000	18.2745728336791	20.2215366221402	20.5580000000000	20.5870411045265	24.7752116335108	25.4440000000000	25.4727784028147	42.2641197325575	44.8100000000000	45.0586254313493
16	1.16478772806060	1.16000000000000	1.16047806391678	6.30455553299530	5.86600000000000	5.91392136520779	9.90901387750200	9.59200000000000	9.53272249601216	17.6122778068676	17.7775000000000	17.7808584773831	19.3660622346573	19.7600000000000	19.7922026100764	24.2367574666447	24.8900000000000	24.9480636376486	42.0488514948797	44.0180000000000	44.1506786374741
17	1.68923622963246	1.64600000000000	1.64855304544952	6.54549202251663	6.02333333333334	6.10318738670951	9.23676688552997	8.45000000000000	8.49123932031090	19.0287421142967	19.5000000000000	19.5196647201670	18.6367477262190	19.0160000000000	19.0259754185391	24.7297311873014	25.4080000000000	25.5106304586597	42.1571871561150	43.4480000000000	43.6264968307135
18	-0.599896172504220	-0.646000000000000	-0.624358297168760	6.34868258419747	5.73400000000000	5.77260576345038	10.2512374923062	9.67800000000000	9.72780718062005	18.1606863181593	18.3725000000000	18.3933378827511	18.8615222515346	19.3160000000000	19.3295636873492	23.0441521310630	23.7840000000000	23.7687388671548	42.7120438641705	43.4180000000000	43.6346642135831
19	-1.28377388059499	-1.59250000000000	-1.47227300915417	6.27850771346432	5.60500000000000	5.62998939946962	10.0609035668404	9.50200000000000	9.49389557221809	16.6404657440454	16.5340000000000	16.5333665924252	19.0334558579714	19.5166666666667	19.5383695574983	23.0203628450902	23.8180000000000	23.7926254165161	43.9794297983592	43.5200000000000	43.6228076937652
20	-0.0786869313852201	-0.198000000000000	-0.168558160589120	5.92838846641032	5.53400000000000	5.69616638448785	7.65481408701074	6.77750000000000	6.82119425946367	17.2677947077791	17.3940000000000	17.3924866112490	19.4004617657799	19.8650000000000	19.8744840361961	22.9379045353463	23.7480000000000	23.7136032835874	41.4416796471860	42.7640000000000	42.8641373937957
21	1.20031071972165	1.02400000000000	1.06254620056320	6.24934893790904	5.74600000000000	5.78686293939237	10.5847180395899	9.93600000000000	10.0248977673760	15.8771823155101	15.7800000000000	15.7783765104898	19.3490752116914	19.9880000000000	20.0188348761750	23.9198426935855	24.5280000000000	24.5176200634035	43.5354404427483	43.7660000000000	43.9646535716393
22	2.96159805467574	2.87400000000000	2.89382077358721	5.82401219838199	5.33500000000000	5.34962569638447	9.82520161425335	9.41800000000000	9.45175754172295	16.2895422008085	16.3450000000000	16.3467703583034	19.3365776905629	19.9440000000000	19.9823850114322	23.5006750289107	24.1720000000000	24.1488268662091	42.1629605127228	43.1780000000000	43.2875557251439
23	2.25422742249320	2.09400000000000	2.14570791902431	6.07726745240039	5.51200000000000	5.55259225414736	8.93134820513446	8.18200000000000	8.28626835522075	17.3369716352182	17.4225000000000	17.4280775374980	19.4574532946181	20.0320000000000	20.0571073546427	24.7209695313054	25.2700000000000	25.2726788158087	42.5829276597007	42.8780000000000	42.9966440347290
24	0.604703175228780	0.564000000000000	0.570300833654660	5.41559900764221	4.89200000000000	4.88150001186074	6.95732189872735	6.27000000000000	6.40292683763575	17.6256446754600	17.8480000000000	17.8548127713491	19.6661744205575	20.4000000000000	20.4377155818873	24.3782538750049	24.8640000000000	24.8596556962002	43.2827885358740	43.5960000000000	43.7844261301612
25	1.42049793475546	1.37400000000000	1.39882769462874	5.50319490154113	4.76333333333334	4.84675981706884	8.96134457472036	8.07200000000000	8.21279973858011	17.0557571300032	17.3380000000000	17.3350242058744	19.4068315600348	20.0340000000000	20.0851662392693	23.5246243757042	23.8140000000000	23.8186355062000	42.4421967392993	43.7820000000000	43.9219344979383
26	0.626146420195280	0.552500000000000	0.564025878066870	4.72019787971117	4.16800000000000	4.24556102999542	8.47718341665901	7.54250000000000	7.71814138770787	16.2384990466884	16.5600000000000	16.5643391936859	20.1227700085956	20.5850000000000	20.6191539244798	27.5263129911308	27.6675000000000	27.6747853857375	42.8711943006097	42.9525000000000	43.0799186758287
27	0.831904237451450	0.780000000000000	0.794614381992220	5.21884140094685	4.49000000000000	4.60557618885877	6.83644503020169	6.18200000000000	6.31595824703115	15.9653257806463	16.2040000000000	16.2010070975840	20.3079935078151	20.8760000000000	20.9589561117751	25.4128046463574	25.6220000000000	25.6167610809008	43.1374811728520	42.9100000000000	43.0299679271563
28	2.06578400352822	1.91250000000000	1.93331684261294	3.52961139245262	3.03500000000000	3.11646960013574	6.26654625954930	5.23200000000000	5.28596078795177	15.8586907104772	16.2766666666667	16.2727127462237	20.4030122827021	20.9425000000000	20.9783766619345	24.7461622176567	24.9366666666667	24.9229731263757	41.0907954595952	43.6920000000000	43.7894813816925
29	0.892732243638600	0.872500000000000	0.861883957280100	3.91108349410762	3.48000000000000	3.44513549858081	6.15036999173437	4.86000000000000	5.16658922375973	15.6552510215022	16.2225000000000	16.2083650788944	20.9510334937436	21.8500000000000	21.9628572877712	27.1739616502583	27.3920000000000	27.4156858150042	42.2048792206908	43.2260000000000	43.3293655830532
30	0.607457267008320	0.498000000000000	0.503512579093510	4.93093791127343	4.44800000000000	4.47682941493742	8.49194312318837	7.45600000000000	7.69563973522468	15.0517461464701	15.5720000000000	15.5535703648020	21.7909382475320	26.8400000000000	25.7471610252634	25.6628397278393	26.3040000000000	26.3880680564139	42.3188227180763	43.2825000000000	43.4170544145208
31	0.713908198768050	0.586666666666660	0.591823945916920	4.16264148893880	3.57400000000000	3.65036637127552	10.0336678069155	8.91600000000000	9.18978671599057	14.4436169021808	14.5225000000000	14.5253285173987	20.4430983322763	20.9900000000000	21.0368378455552	26.4755700329300	26.9850000000000	27.0408724426861	42.6640227268578	42.7933333333333	42.9049692324850
32	1.54542326525275	1.44200000000000	1.46002338857980	4.08319088034771	3.02333333333333	3.23129135010971	9.70355238046224	8.72000000000000	8.84913632991041	14.9074370922597	15.4880000000000	15.5011096596430	20.5928908566394	21.1633333333333	21.1477328725167	24.4443379486085	24.8220000000000	24.8608273915363	41.1669987279124	43.0700000000000	43.3662086549097
33	0.963180141079080	0.796666666666670	0.836165606035350	3.93500200101512	2.65666666666667	2.96196202402082	8.82657938753860	8.04400000000000	8.09736460644642	14.1070945701059	14.4975000000000	14.4961614829945	20.8575184625413	21.3950000000000	21.4642834155967	23.9556734035920	24.3880000000000	24.3957366601395	41.0740184311441	42.4720000000000	42.6968538723723
34	0.541239846506750	0.554000000000000	0.554781122557700	4.55230378051570	3.49250000000000	3.67672099929097	8.51321970468605	7.71000000000000	7.83598261917490	13.8134344422451	14.5580000000000	14.5711264948338	20.5230571280776	21.1240000000000	21.1769861137136	25.4140511017675	25.8860000000000	25.9068075548221	39.5051089393237	48.2550000000000	47.7587403732441
35	0.717818696756940	0.690000000000000	0.691435257371750	3.53152115477557	2.84666666666667	2.96808350133810	9.00520536388359	8.17800000000000	8.33844556230296	15.1703639184943	15.9600000000000	15.9576613992542	20.3170013731613	20.9280000000000	20.9670363109910	25.7511356076313	26.2540000000000	26.3692476413042	41.5930307348605	42.8325000000000	42.8558700002784
36	-0.960730595180070	-1.09500000000000	-1.06139898146338	4.48852116326464	3.86800000000000	4.00759272590173	9.57392597710082	9.08500000000000	9.14260612849853	15.8384716842659	16.3900000000000	16.3166358684866	19.9362440279872	20.4900000000000	20.5127083469160	24.0525329475202	24.2725000000000	24.2838612499147	41.4014777512068	42.8200000000000	42.8937714536426
37	-0.220764710059230	-0.386000000000000	-0.358191012773250	4.09467351441234	3.51800000000000	3.59272377707801	9.78196933642702	9.16000000000000	9.24673755181553	16.0967788653795	16.5575000000000	16.5546478637201	18.9578620077326	19.6475000000000	19.6630020632943	25.1425381284459	25.6500000000000	25.6680879841402	41.7080736733470	43.1980000000000	43.3180809179150
38	0.496346341203740	0.352000000000000	0.368259507133380	4.02623832045302	3.63800000000000	3.81776673035489	9.36354421540602	8.64800000000000	8.71551707558267	16.0657158590156	16.3175000000000	16.3101636715451	18.8501012946207	19.4725000000000	19.5267787100462	25.8187068416270	26.5520000000000	26.5859245647516	41.6428402083272	43.2425000000000	43.3868278793321
39	0.163247706265610	-0.00249999999999995	0.0300092679179000	4.50561577569320	3.99666666666667	4.02715641464342	8.00651091735603	7.34600000000000	7.37463793006023	15.3107534067000	15.5800000000000	15.5746578102670	19.2986538066520	19.7600000000000	19.7917910614634	25.0904633483808	25.8440000000000	25.8315289171430	40.5735235072116	43.6725000000000	43.8491301076825
40	-0.0385802667235999	-0.132000000000000	-0.0718308654058699	3.38843786097079	2.90500000000000	3.09278140925788	7.47341541904982	6.49750000000000	6.59532639689645	16.0353667233838	16.3060000000000	16.3044559444962	19.3147821574759	19.7040000000000	19.7265522992112	27.0216656571760	27.4460000000000	27.4598488119508	43.1233983239263	43.2600000000000	43.4632734020752
41	2.00663076129142	1.98600000000000	1.99621122455157	4.46129785335133	3.85400000000000	4.00769090131713	9.03264429262460	8.24800000000000	8.32773457364549	16.7754421999310	17.0320000000000	17.0275812969759	19.4484453509744	19.8040000000000	19.8345666630969	26.1410396257458	26.7880000000000	26.7893065227971	42.6000718091686	43.4440000000000	43.6126958612419
42	0.569229212425920	0.570000000000000	0.567663456917610	3.89846847765784	3.50000000000000	3.66660508393474	9.59723478198528	8.74200000000000	8.75669516810875	16.3027248969158	16.6600000000000	16.6593135476352	19.6437793964322	20.1020000000000	20.1468236794796	25.5945062517842	26.5560000000000	26.5562936470916	41.8203028625969	42.9700000000000	43.2349153180203
43	0.210210837141070	0.147499999999990	0.148393542202270	5.96836872326137	5.63200000000000	5.65178029784975	10.9304889106127	9.88000000000000	9.99002556100613	16.2093950615780	16.7860000000000	16.7784014852397	19.2273713809079	20.0460000000000	20.1115178782714	24.0135795231476	24.9360000000000	24.9417847799886	41.7031413954748	43.1240000000000	43.2388587973728
44	0.536894360900450	0.486000000000000	0.490792794564200	5.45801935864307	4.85500000000000	4.88509650450425	10.9600799680860	9.57800000000000	9.93840355276449	15.9073465941809	16.2220000000000	16.2192834236814	19.7397295388121	20.3500000000000	20.3454413360696	25.0944001918607	25.5620000000000	25.5593872312065	42.5810373556514	43.1100000000000	43.1893934349878
45	-0.571609599355780	-0.584000000000000	-0.585048506485110	6.55151230398573	5.92800000000000	5.95239770876939	10.4094476923379	9.25200000000000	9.60644056397185	16.6400645031299	17.0500000000000	17.0301476745389	20.4446715513205	21.0900000000000	21.1497831143132	24.0686332893050	24.9375000000000	24.9653928154419	42.7950955046047	43.2740000000000	43.3626414298355
46	-0.762656403041950	-0.750000000000000	-0.752331128513420	5.34285380761153	4.66200000000000	4.73022481094170	9.66479714867075	8.31600000000000	8.43875485686107	16.7344102414901	17.1620000000000	17.1461807590604	20.1735490100805	20.5950000000000	20.6420829564410	24.3605643325213	25.2260000000000	25.2043037507171	41.9398099514873	43.2600000000000	43.3970265611989
47	0.0620904158577198	0.0299999999999998	0.0303699239133199	6.02548196942445	5.50400000000000	5.55190653372526	6.95615342732864	6.01000000000000	6.44023465840079	15.6515811775195	16.0740000000000	16.0710103876506	20.2001697830914	20.5850000000000	20.6158123862776	24.2890580434002	25.1240000000000	25.1163025574497	42.6740197502529	43.3860000000000	43.4403739196187
48	1.28687715217480	1.36200000000000	1.36040299729997	4.50822071067094	4.09000000000000	4.05757406031418	8.44407351982170	7.07250000000000	7.41538208137726	15.5770134856791	16.0360000000000	16.0337370858734	20.3065178693454	20.6280000000000	20.6585673544296	23.6471386580102	24.5880000000000	24.5676583045533	41.9611503869706	43.5720000000000	43.6238533100196
49	0.628420878626580	0.638000000000000	0.638095029634210	6.35018237427595	5.88200000000000	5.88706715096878	7.84812858529248	6.94000000000000	7.01878935778907	15.7116655013175	16.1833333333333	16.1882194960341	20.5517252324829	20.8340000000000	20.8618963278783	23.9964247314568	24.7220000000000	24.7272523812164	41.2798447705717	43.3020000000000	43.4922090430925
50	1.31239402533967	1.28400000000000	1.28601306259196	6.07671772246573	5.79000000000001	5.79528941073341	8.04356481764499	7.29000000000000	7.34516806837962	16.7217866449853	17.1840000000000	17.2262383915728	21.1480290098558	21.4880000000000	21.5143922243653	23.0977400299106	24.1460000000000	24.1721176319596	43.0611326620349	43.4975000000000	43.7520039402645
51	1.40107491291832	1.37600000000000	1.37489286023005	6.03011923513691	5.57000000000000	5.59910593129219	8.28948842755975	7.20600000000000	7.38831618771188	16.6839543106914	17.1160000000000	17.1183124653734	21.0641316187327	21.4420000000000	21.4817435046169	23.6925166392478	24.3775000000000	24.3892598162187	42.4403405123991	42.8925000000000	43.2970655917547
52	2.46928650718815	2.44800000000000	2.44869076096791	6.64287206108669	6.37800000000000	6.40028138620113	8.72128759471076	7.51750000000001	7.67522375910552	16.1511839229463	16.3940000000000	16.3990383428658	21.4299774519424	21.7960000000000	21.8003291895877	22.7372145118200	23.4440000000000	23.4586115760157	41.8860603896274	43.2225000000000	43.9417804489377
53	2.43171840786894	2.39250000000000	2.39792405007908	5.92048846721097	5.34400000000000	5.41866435692529	8.29675278776300	7.03400000000000	7.37914994537606	15.2917441045585	15.7825000000000	15.7593238962563	20.6790372367301	21.1240000000000	21.1258871224944	23.9193462183764	24.7760000000000	24.7925693782390	40.8678053365056	43.0280000000000	43.5990556113078
54	2.06814934710960	2.06400000000000	2.06483379150127	7.34600549074150	6.86400000000000	6.90495746842841	10.4863929287274	9.45200000000000	9.61014529989648	13.7189758390086	14.0960000000000	14.0738719708564	21.1687180237661	21.7200000000000	21.7275443929943	23.3640795349693	24.1980000000000	24.1935254648045	41.2209759203072	42.9060000000000	43.4922389643326
55	3.10263399994352	3.11666666666666	3.07547033726902	5.06526455944631	4.59600000000000	4.66082353178937	10.3690231648906	9.38600000000000	9.58254136616546	14.8159609497669	14.8680000000000	14.8719873426141	20.9298825962970	21.4480000000000	21.4637403124129	24.3829021386241	24.8600000000000	24.8880674565115	41.9013309607227	43.8350000000000	44.4661889725364
56	2.86086985605299	2.86750000000000	2.87012300868671	7.07298823248931	6.50800000000000	6.62338274548767	11.5322424566013	10.3440000000000	10.5685302880189	16.3985313386878	16.2700000000000	16.2684345447444	20.1502345444568	20.5750000000000	20.5887491596239	24.1202815544671	24.6180000000000	24.6555397271457	40.7841454267947	42.1380000000000	42.5052059872840
57	2.34393201488572	2.37000000000000	2.37240204155129	5.18603708388851	4.84400000000000	4.89386615980606	11.5028862454883	10.8020000000000	10.9210258010207	16.3581837783159	16.3200000000000	16.3243988469094	20.3311891443150	20.6580000000000	20.6671490216697	24.0271177521134	24.6066666666667	24.5932718097304	42.4189995723750	43.5560000000000	44.0694000497864
58	0.802252109668870	0.566000000000000	0.601203511200560	4.85295289946595	4.09600000000000	4.15264999017717	11.2637830729968	10.6980000000000	10.7402203410155	17.1210840933179	16.9825000000000	16.9677287728430	20.8681743962090	21.1920000000000	21.1940118824824	23.8171376184861	24.1166666666667	24.1456094625389	38.8569343270746	43.5920000000000	44.5116190933476
59	-0.960345500442170	-1.01400000000000	-0.995484623324990	4.44853653404110	3.89000000000000	3.93371673101933	11.2220134779378	10.5900000000000	10.6170448397483	18.6508073478398	18.5175000000000	18.4788783000329	20.9435827843982	21.0960000000000	21.0973682565309	25.1873137650793	25.7100000000000	25.7883577322663	35.2307437445062	44.7200000000000	45.9395496676239
60	-0.795855334498700	-0.952000000000000	-0.931806731691410	3.81177538245037	3.02400000000000	3.08070353067109	9.95198374394410	9.28000000000000	9.28066744760247	16.1139660862429	16.1400000000000	16.1403034254654	20.8720408531170	21.2780000000000	21.2754170236440	22.8346127840515	23.3300000000000	23.3919063169706	34.7687702198290	42.4150000000000	42.9999296070326
